New constraints on oscillation parameters from $\nu_e$ appearance and $\nu_\mu$ disappearance in the NOvA experiment

We present updated results from the NOvA experiment for $\nu_\mu\rightarrow\nu_\mu$ and $\nu_\mu\rightarrow\nu_e$ oscillations from an exposure of $8.85\times10^{20}$ protons on target, which represents an increase of 46% compared to our previous publication. The results utilize significant improvements in both the simulations and analysis of the data. A joint fit to the data for $\nu_\mu$ disappearance and $\nu_e$ appearance gives the best fit point as normal mass hierarchy, $\Delta m^2_{32} = 2.44\times 10^{-3}{{\rm eV}^2}/c^4$, $\sin^2\theta_{23} = 0.56$, and $\delta_{CP} = 1.21\pi$. The 68.3% confidence intervals in the normal mass hierarchy are $\Delta m^2_{32} \in [2.37,2.52]\times 10^{-3}{{\rm eV}^2}/c^4$, $\sin^2\theta_{23} \in [0.43,0.51] \cup [0.52,0.60]$, and $\delta_{CP} \in [0,0.12\pi] \cup [0.91\pi,2\pi]$. The inverted mass hierarchy is disfavored at the 95% confidence level for all choices of the other oscillation parameters.

==> 9e20 submission draft/novacurrent18.tex <==
%voffset documentclass[prd,superscriptaddress]{revtex4}
%\% 0.5in 
%\usepackage{graphicx}% Include figure files
%\usepackage{dcolumn}% Align table columns on decimal point
%\usepackage{bm}% bold math
%\%begin{document}
%\title{Updated constraints on oscillation parameters from
%$\nu_e$ appearance and $\nu_\mu$ disappearance in NOvA}
%NOvA Current Author List
%last Version 23 April 2018, Maintained by Maury Goodman
\newcommand{\ANL}{Argonne National Laboratory, Argonne, Illinois 60439, 
USA}
\newcommand{\ICS}{Institute of Computer Science, The Czech 
Academy of Sciences, 
182 07 Prague, Czech Republic}
\newcommand{\IOP}{Institute of Physics, The Czech 
Academy of Sciences, 
182 21 Prague, Czech Republic}
%\newcommand{\Athens}{Department of Physics, University of Athens, 
%Athens, 15771, Greece}
\newcommand{\Atlantico}{Universidad del Atlantico,
Km. 7 antigua via a Puerto Colombia, Barranquilla, Colombia}
\newcommand{\BHU}{Department of Physics, Institute of Science, Banaras 
Hindu University, Varanasi, 221 005, India}
\newcommand{\UCLA}{Physics and Astronomy Department, UCLA, Box 951547, Los 
Angeles, California 90095-1547, USA}
\newcommand{\Caltech}{California Institute of 
Technology, Pasadena, California 91125, USA}
\newcommand{\Cochin}{Department of Physics, Cochin University
of Science and Technology, Kochi 682 022, India}
\newcommand{\Charles}
{Charles University, Faculty of Mathematics and Physics,
 Institute of Particle and Nuclear Physics, Prague, Czech Republic}
\newcommand{\Cincinnati}{Department of Physics, University of Cincinnati, 
Cincinnati, Ohio 45221, USA}
\newcommand{\CSU}{Department of Physics, Colorado 
State University, Fort Collins, CO 80523-1875, USA}
\newcommand{\CTU}{Czech Technical University in Prague,
Brehova 7, 115 19 Prague 1, Czech Republic}
\newcommand{\Dallas}{Physics Department, University of Texas at Dallas,
800 W. Campbell Rd. Richardson, Texas 75083-0688, USA}
\newcommand{\Delhi}{Department of Physics and Astrophysics, University of 
Delhi, Delhi 110007, India}
\newcommand{\JINR}{Joint Institute for Nuclear Research,  
Dubna, Moscow region 141980, Russia}
\newcommand{\FNAL}{Fermi National Accelerator Laboratory, Batavia, 
Illinois 60510, USA}
\newcommand{\UFG}{Instituto de F\'{i}sica, Universidade Federal de 
Goi\'{a}s, Goi\^{a}nia, Goi\'{a}s, 74690-900, Brazil}
\newcommand{\Guwahati}{Department of Physics, IIT Guwahati, Guwahati, 781 
039, India}
\newcommand{\Harvard}{Department of Physics, Harvard University, 
Cambridge, Massachusetts 02138, USA}
\newcommand{\Houston}{Department of Physics, 
University of Houston, Houston, Texas 77204, USA}
\newcommand{\IHyderabad}{Department of Physics, IIT Hyderabad, Hyderabad, 
502 205, India}
\newcommand{\Hyderabad}{School of Physics, University of Hyderabad, 
Hyderabad, 500 046, India}
\newcommand{\IIT}{Department of Physics,
Illinois Institute of Technology,
Chicago IL 60616, USA}
\newcommand{\Indiana}{Indiana University, Bloomington, Indiana 47405, 
USA}
\newcommand{\INR}{Inst. for Nuclear Research of Russia, Academy of 
Sciences 7a, 60th October Anniversary prospect, Moscow 117312, Russia}
\newcommand{\Iowa}{Department of Physics and Astronomy, Iowa State 
University, Ames, Iowa 50011, USA}
\newcommand{\Irvine}{Department of Physics and Astronomy, 
University of California at Irvine, Irvine, California 92697, USA}
\newcommand{\Jammu}{Department of Physics and Electronics, University of 
Jammu, Jammu Tawi, 180 006, Jammu and Kashmir, India}
\newcommand{\Lebedev}{Nuclear Physics and Astrophysics Division, Lebedev 
Physical 
Institute, Leninsky Prospect 53, 119991 Moscow, Russia}
\newcommand{\MSU}{Department of Physics and Astronomy, Michigan State 
University, East Lansing, Michigan 48824, USA}
\newcommand{\Duluth}{Department of Physics and Astronomy, 
University of Minnesota Duluth, Duluth, Minnesota 55812, USA}
\newcommand{\Minnesota}{School of Physics and Astronomy, University of 
Minnesota Twin Cities, Minneapolis, Minnesota 55455, USA}
\newcommand{\Oxford}{Subdepartment of Particle Physics, 
University of Oxford, Oxford OX1 3RH, United Kingdom}
\newcommand{\Panjab}{Department of Physics, Panjab University, 
Chandigarh, 106 014, India}
\newcommand{\Pitt}{Department of Physics, 
University of Pittsburgh, Pittsburgh, Pennsylvania 15260, USA}
\newcommand{\RAL}{Rutherford Appleton Laboratory, Science and 
Technology Facilities Council, Didcot, OX11 0QX, United Kingdom}
\newcommand{\SAlabama}{Department of Physics, University of 
South Alabama, Mobile, Alabama 36688, USA} 
\newcommand{\Carolina}{Department of Physics and Astronomy, University of 
South Carolina, Columbia, South Carolina 29208, USA}
\newcommand{\SDakota}{South Dakota School of Mines and Technology, Rapid 
City, South Dakota 57701, USA}
\newcommand{\SMU}{Department of Physics, Southern Methodist University, 
Dallas, Texas 75275, USA}
\newcommand{\Stanford}{Department of Physics, Stanford University, 
Stanford, California 94305, USA}
\newcommand{\Sussex}{Department of Physics and Astronomy, University of 
Sussex, Falmer, Brighton BN1 9QH, United Kingdom}
\newcommand{\Syracuse}{Department of Physics, Syracuse University,
Syracuse NY 13210, USA}
\newcommand{\Tennessee}{Department of Physics and Astronomy, 
University of Tennessee, Knoxville, Tennessee 37996, USA}
\newcommand{\Texas}{Department of Physics, University of Texas at Austin, 
Austin, Texas 78712, USA}
\newcommand{\Tufts}{Department of Physics and Astronomy, Tufts University, Medford, 
Massachusetts 02155, USA}
\newcommand{\UCL}{Physics and Astronomy Dept., University College London, 
Gower Street, London WC1E 6BT, United Kingdom}
\newcommand{\Virginia}{Department of Physics, University of Virginia, 
Charlottesville, Virginia 22904, USA}
\newcommand{\WSU}{Department of Mathematics, Statistics, and Physics,
 Wichita State University, 
Wichita, Kansas 67206, USA}
\newcommand{\WandM}{Department of Physics, College of William \& Mary, 
Williamsburg, Virginia 23187, USA}
\newcommand{\Winona}{Department of Physics, Winona State University, P.O. 
Box 5838, Winona, Minnesota 55987, USA}
\newcommand{\Crookston}{Math, Science and Technology Department, University 
of Minnesota -- Crookston, Crookston, Minnesota 56716, USA}
\newcommand{\deceased}{Deceased.}

\affiliation{\ANL}
\affiliation{\Atlantico}
%\affiliation{\Athens}
\affiliation{\BHU}
%\affiliation{\UCLA}
\affiliation{\Caltech}
\affiliation{\Charles}
\affiliation{\Cincinnati}
\affiliation{\Cochin}
\affiliation{\CSU}
\affiliation{\CTU}
\affiliation{\Delhi}
\affiliation{\FNAL}
\affiliation{\UFG}
\affiliation{\Guwahati}
\affiliation{\Harvard}
\affiliation{\Hyderabad}
\affiliation{\IHyderabad}
\affiliation{\Indiana}
\affiliation{\ICS}
\affiliation{\IIT}
\affiliation{\INR}
\affiliation{\IOP}
\affiliation{\Iowa}
\affiliation{\Irvine}
\affiliation{\Jammu}
\affiliation{\JINR}
\affiliation{\Lebedev}
\affiliation{\MSU}
%\affiliation{\Crookston}
\affiliation{\Duluth}
\affiliation{\Minnesota}
%\affiliation{\Oxford}
\affiliation{\Panjab}
%\affiliation{\RAL}
\affiliation{\SAlabama}
\affiliation{\Carolina}
\affiliation{\SDakota}
\affiliation{\SMU}
\affiliation{\Stanford}
\affiliation{\Sussex}
\affiliation{\Syracuse}
\affiliation{\Tennessee}
\affiliation{\Texas}
%\affiliation{\Dallas}
\affiliation{\Tufts}
\affiliation{\UCL}
\affiliation{\Virginia}
\affiliation{\WSU}
\affiliation{\WandM}
\affiliation{\Winona}



%Added June 2017
\author{M.~A.~Acero}
\affiliation{\Atlantico}

\author{P.~Adamson}
\affiliation{\FNAL}

%For first publication
%\author{C.~Ader}
%\affiliation{\FNAL}

%Added March 2017
\author{L.~Aliaga}
\affiliation{\FNAL}

\author{T.~Alion}
\affiliation{\Sussex}

\author{V.~Allakhverdian}
\affiliation{\JINR}

%Legacy June 2017
%\author{D.~Ambrose}
%\affiliation{\Minnesota}

%For first publication
%\author{M.~Andrews}
%\affiliation{\FNAL}

\author{N.~Anfimov}
\affiliation{\JINR}

%Went Legacy 1 Feb 2016
%\author{I.~Anghel}
%\affiliation{\Iowa}
%\affiliation{\ANL}

\author{A.~Antoshkin}
\affiliation{\JINR}

%For first publication
%\author{K.~Arms}
\affiliation{\Minnesota}

% Legacy June 2017 opted in
\author{E.~Arrieta-Diaz}
\affiliation{\SMU}

%Removed June 2017
%\author{K.~Augsten}
%\affiliation{\CTU}


\author{A.~Aurisano}
\affiliation{\Cincinnati}

%For first publication
%\author{D.~S.~Ayres}
%\affiliation{\ANL}

\author{A.~Back}
\affiliation{\Iowa}

\author{C.~Backhouse}
\affiliation{\UCL}

\author{M.~Baird}
\affiliation{\Indiana}
\affiliation{\Sussex}
\affiliation{\Virginia}

\author{N.~Balashov}
\affiliation{\JINR}

\author{B.~A.~Bambah}
\affiliation{\Hyderabad}

\author{K.~Bays}
\affiliation{\Caltech}

\author{B.~Behera}
\affiliation{\IHyderabad}

\author{S.~Bending}
\affiliation{\UCL}

\author{R.~Bernstein}
\affiliation{\FNAL}

%For first publication
%\author{M.~Betancourt}
%\affiliation{\Minnesota}

\author{V.~Bhatnagar}
\affiliation{\Panjab}

\author{B.~Bhuyan}
\affiliation{\Guwahati}

\author{J.~Bian}
\affiliation{\Irvine}
\affiliation{\Minnesota}

%For first publication
%\author{K.~Biery}
%\affiliation{\FNAL}

\author{T.~Blackburn}
\affiliation{\Sussex}

%For first publication
%\author{V.~Bocean}
%\affiliation{\FNAL}

%For first publication
%\author{D.~Bogert}
%\affiliation{\FNAL}

\author{J.~Blair}
\affiliation{\Houston}

\author{A.~Bolshakova}
\affiliation{\JINR}

%Added June 2017
\author{P.~Bour}
\affiliation{\CTU}

%For first publication
%\author{M.~Bowden}
%\affiliation{\FNAL}

%For first publication
%\author{C.~Bower}
%\affiliation{\Indiana}

%For first publication
%\author{D.~Broemmelsiek}
%\affiliation{\FNAL}

\author{C.~Bromberg}
\affiliation{\MSU}

\author{J.~Brown}
\affiliation{\Minnesota}

% Legacy June 2017
%\author{G.~Brunetti}
%\affiliation{\FNAL}

% Went legacy August 2016
%\author{X.~Bu}
%\affiliation{\FNAL}

\author{N.~Buchanan}
\affiliation{\CSU}

\author{A.~Butkevich}
\affiliation{\INR}

\author{V.~Bychkov}
\affiliation{\Minnesota}

\author{M.~Campbell}
\affiliation{\UCL}

%For first publication
%\author{D.~Capista}
%\affiliation{\FNAL}

\author{T.~J.~Carroll}
\affiliation{\Texas}

\author{E.~Catano-Mur}
\affiliation{\Iowa}

\author{A.~Cedeno}
\affiliation{\WSU}

%For first publication
%\author{T.~R.~Chase}
%\affiliation{\Minnesota}

\author{S.~Childress}
\affiliation{\FNAL}

\author{B.~C.~Choudhary}
\affiliation{\Delhi}

\author{B.~Chowdhury}
\affiliation{\Carolina}

\author{T.~E.~Coan}
\affiliation{\SMU}

%Went Legacy 1 Feb 2016
%\author{J.~A.~B.~Coelho}
%\affiliation{\Tufts}

\author{M.~Colo}
\affiliation{\WandM}

%Went Legacy 1 Jan 2018 opted in
\author{J.~Cooper}
\affiliation{\FNAL}

\author{L.~Corwin}
\affiliation{\SDakota}

\author{L.~Cremonesi}
\affiliation{\UCL}

\author{D.~Cronin-Hennessy}
\affiliation{\Minnesota}

%For first publication
%Remember to remove Dallas
%\author{A.~Cunningham}
%\affiliation{\Dallas}

\author{G.~S.~Davies}
\affiliation{\Indiana}

% Legacy June 2017 opted in
\author{J.~P.~Davies}
\affiliation{\Sussex}

\author{S.~De~Rijck}
\affiliation{\Texas}

%For first publication
%\author{M.~Del~Tutto}
%\affiliation{\FNAL}

\author{P.~F.~Derwent}
\affiliation{\FNAL}

%First publication only
%\author{K.~N.~Deepthi}
%\affiliation{\Hyderabad}

%For first publication
%Remember to remove Crookston
%\author{D.~Demuth}
%\affiliation{\Crookston}

% Went legacy August 2016
%\author{S.~Desai}
%\affiliation{\Minnesota}

%For first publication
%\author{G.~Deuerling}
%\affiliation{\FNAL}

%For first publication
%\author{A.~Devan}
%\affiliation{\WandM}

%For first publication
%\author{J.~Dey}
%\affiliation{\FNAL}

\author{R.~Dharmapalan}
\affiliation{\ANL}

\author{P.~Ding}
\affiliation{\FNAL}

%For first publication
%\author{S.~Dixon}
%\affiliation{\FNAL}

\author{Z.~Djurcic}
\affiliation{\ANL}

\author{E.~C.~Dukes}
\affiliation{\Virginia}

\author{P.~Dung}
\affiliation{\Texas}

\author{H.~Duyang}
\affiliation{\Carolina}

%For first publication
%\author{Y.~Efremenko}
%\affiliation{\Tennessee}

\author{S.~Edayath}
\affiliation{\Cochin}

\author{R.~Ehrlich}
\affiliation{\Virginia}

\author{G.~J.~Feldman}
\affiliation{\Harvard}

%For first publication
%\author{N.~Felt}
%\affiliation{\Harvard}

%For first publication
%\author{E.~J.~Fenyves}
%\altaffiliation{\deceased}
%\affiliation{\Dallas}

%For first publication
%\author{E.~Flumerfelt}
%\affiliation{\Tennessee}

%For first publication
%\author{S.~Foulkes}
%\affiliation{\FNAL}

% Went legacy August 2016; Rejoined September 2016
\author{M.~J.~Frank}
\affiliation{\SAlabama}
\affiliation{\Virginia}

%For first publication
%\author{W.~Freeman}
%\affiliation{\FNAL}

% Legacy June 2017
%\author{M.~Gabrielyan}
%\affiliation{\Minnesota}

\author{H.~R.~Gallagher}
\affiliation{\Tufts}

\author{R.~Gandrajula}
\affiliation{\MSU}

\author{F.~Gao}
\affiliation{\Pitt}

\author{S.~Germani}
\affiliation{\UCL}

%For first publication
%\author{M.~Gebhard}
%\affiliation{\Indiana}

%Went Legacy 1 Jan 2018
%\author{T.~Ghosh}
%\affiliation{\UFG}

%For first publication
%\author{W.~Gilbert}
%\affiliation{\Minnesota}

\author{A.~Giri}
\affiliation{\IHyderabad}

%For first publication
%\author{S.~Goadhouse}
%\affiliation{\Virginia}

\author{R.~A.~Gomes}
\affiliation{\UFG}

%For first publication
%\author{L.~Goodenough}
%\affiliation{\ANL}

\author{M.~C.~Goodman}
\affiliation{\ANL}

\author{V.~Grichine}
\affiliation{\Lebedev}

%Added March 2017
\author{M.~Groh}
\affiliation{\Indiana}

%For first publication
%\author{N.~Grossman}
%\affiliation{\FNAL}

\author{R.~Group}
\affiliation{\Virginia}

%Went Legacy 1 January 2018
\author{D.~Grover}
\affiliation{\BHU}

%For first publication
%\author{J.~Grudzinski}
%\affiliation{\ANL}

%For first publication
%\author{V.~Guarino}
%\affiliation{\ANL}

\author{B.~Guo}
\affiliation{\Carolina}

\author{A.~Habig}
\affiliation{\Duluth}

\author{F.~Hakl}
\affiliation{\ICS}

%Went Legacy 1 Feb 2016
%\author{T.~Handler}
%\affiliation{\Tennessee}

\author{J.~Hartnell}
\affiliation{\Sussex}

\author{R.~Hatcher}
\affiliation{\FNAL}

\author{A.~Hatzikoutelis}
\affiliation{\Tennessee}

\author{K.~Heller}
\affiliation{\Minnesota}

\author{A.~Himmel}
\affiliation{\FNAL}

\author{A.~Holin}
\affiliation{\UCL}

%Added March 2017
\author{B.~Howard}
\affiliation{\Indiana}

\author{J.~Huang}
\affiliation{\Texas}

\author{J.~Hylen}
\affiliation{\FNAL}

%For first publication
%\author{C.~Howcroft}
%\affiliation{\Caltech}

%For first publication
%\author{J.~Huang}
%\affiliation{\Texas}

%For first publication
%\author{X.~Huang}
%\affiliation{\ANL}

%For first publication
%\author{J.~Hylen}
%\affiliation{\FNAL}

%For first publication
%\author{M.~Ishitsuka}
%\affiliation{\Indiana}

\author{F.~Jediny}
\affiliation{\CTU}

% Removed December 2016
%\author{Z.~Jelinkova}
%\affiliation{\Charles}


%For first publication
%\author{C.~Jensen}
%\affiliation{\FNAL}


%For first publication
%\author{D.~Jensen}
%\affiliation{\FNAL}

%For first publication
%\author{C.~Johnson}
%\affiliation{\Indiana}


%For first publication
%\author{H.~Jostlein}
%\affiliation{\FNAL}

\author{M.~Judah}
\affiliation{\CSU}

% Went legacy August 2016
%\author{G.~K.~Kafka}
%\affiliation{\Harvard}

\author{I.~Kakorin}
\affiliation{\JINR}

\author{D.~Kalra}
\affiliation{\Panjab}

%For first publication
%\author{Y.~Kamyshkov}
%\affiliation{\Tennessee}

\author{D.M.~Kaplan}
\affiliation{\IIT}

% Legacy June 2017
%\author{S.~M.~S.~Kasahara}
%\affiliation{\Minnesota}

%Went Legacy 1 January 2018
%\author{S.~Kasetti}
%\affiliation{\Hyderabad}

\author{R.~Keloth}
\affiliation{\Cochin}

%For first publication
%\author{K.~Kephart}
%\affiliation{\FNAL}

\author{O.~Klimov}
\affiliation{\JINR}

\author{L.W.~Koerner}
\affiliation{\Houston}

%For first publication
%\author{G.~Koizumi}
%\affiliation{\FNAL}

\author{L.~Kolupaeva}
\affiliation{\JINR}

\author{S.~Kotelnikov}
\affiliation{\Lebedev}

\author{I.~Kourbanis}
\affiliation{\FNAL}

%For first publication
%\author{Z.~Krahn}
%\affiliation{\Minnesota}

%For first publication
%\author{V.~Kravtsov}
%\affiliation{\SMU}

\author{A.~Kreymer}
\affiliation{\FNAL}

%For First Publication
%added to author list 2018
\author{Ch.~Kulenberg}
\affiliation{\JINR}

\author{A.~Kumar}
\affiliation{\Panjab}

% Legacy June 2017
%\author{S.~Kurbanov}
%\affiliation{\Virginia}

\author{C.~Kuruppu}
\affiliation{\Carolina}

\author{V.~Kus}
\affiliation{\CTU}

%For first publication
%\author{T.~Kutnink}
%\affiliation{\Iowa}

%For first publication
%\author{R.~Kwarciancy}
%\affiliation{\FNAL}

%For first publication
%\author{J.~Kwong}
%\affiliation{\Minnesota}

% Added March 2017
\author{T.~Lackey}
\affiliation{\Indiana}

\author{K.~Lang}
\affiliation{\Texas}

%For first publication
%\author{A.~Lee}
%\affiliation{\FNAL}

% Went legacy August 2016; opted in until September 2017
%\author{W.~M.~Lee}
%\altaffiliation{\deceased}
%\affiliation{\FNAL}

%For first publication
%Remember to remove UCLA
%\author{K.~Lee}
%\affiliation{\UCLA}

% Went legacy August 2016
%\author{S.~Lein}
%\affiliation{\Minnesota}

%For first publication
%\author{P.~Litchfield}
%\affiliation{\Minnesota}

\author{S.~Lin}
\affiliation{\CSU}

%Went Legacy 1 Feb 2016
%\author{J.~Liu}
%\affiliation{\WandM}

\author{M.~Lokajicek}
\affiliation{\IOP}

\author{J.~Lozier}
\affiliation{\Caltech}

%For first publication
%\author{Q.~Lu}
%\affiliation{\FNAL}

%For first publication
%\author{P.~Lucas}
%\affiliation{\FNAL}

\author{S.~Luchuk}
\affiliation{\INR}

%For first publication
%\author{P.~Lukens}
%\affiliation{\FNAL}

%For first publication
%\author{G.~Lukhanin}
%\affiliation{\FNAL}

\author{K.~Maan}
\affiliation{\Panjab}

\author{S.~Magill}
\affiliation{\ANL}

\author{W.~A.~Mann}
\affiliation{\Tufts}

\author{M.~L.~Marshak}
\affiliation{\Minnesota}


%For first publication
%\author{M.~Martens}
%\affiliation{\FNAL}

%For first publication
%\author{J.~Martincik}
%\affiliation{\CTU}

%Went Legacy 1 Feb 2016
%\author{P.~Mason}
%\affiliation{\Tennessee}

% Legacy June 2017
%\author{K.~Matera}
%\affiliation{\FNAL}

%For first publication
%\author{M.~Mathis}
%\affiliation{\WandM}

\author{V.~Matveev}
\affiliation{\INR}

%For first publication
%\author{N.~Mayer}
%\affiliation{\Tufts}

%For first publication
%\author{E.~McCluskey}
%\affiliation{\FNAL}

%For first publication
%\author{R.~Mehdiyev}
%\affiliation{\Texas}

\author{D. P.~M\'endez}
\affiliation{\Sussex}

%Went Legacy 1 Feb 2016
%\author{H.~Merritt}
%\affiliation{\Indiana}

\author{M.~D.~Messier}
\affiliation{\Indiana}

\author{H.~Meyer}
\affiliation{\WSU}

\author{T.~Miao}
\affiliation{\FNAL}

%For first publication
%\author{D.~Michael}
%\altaffiliation{\deceased}
%\affiliation{\Caltech}


%For first publication
%\author{S.~P.~~Mikheyev}
%\altaffiliation{\deceased}
%\affiliation{\INR}

\author{W.~H.~Miller}
\affiliation{\Minnesota}

\author{S.~R.~Mishra}
\affiliation{\Carolina}

\author{A.~Mislivec}
\affiliation{\Minnesota}

\author{R.~Mohanta}
\affiliation{\Hyderabad}

%For first publication; remade current Feb 2017
\author{A.~Moren}
\affiliation{\Duluth}

\author{L.~Mualem}
\affiliation{\Caltech}

\author{M.~Muether}
\affiliation{\WSU}

\author{S.~Mufson}
\affiliation{\Indiana}

\author{R.~Murphy}
\affiliation{\Indiana}

\author{J.~Musser}
\affiliation{\Indiana}

\author{D.~Naples}
\affiliation{\Pitt}

\author{N.~Nayak}
\affiliation{\Irvine}

%For first publication
%\author{H.~B.~Newman}
%\affiliation{\Caltech}

\author{J.~K.~Nelson}
\affiliation{\WandM}

\author{R.~Nichol}
\affiliation{\UCL}

\author{E.~Niner}
%\affiliation{\Indiana}
\affiliation{\FNAL}

\author{A.~Norman}
\affiliation{\FNAL}

%added December 2016
\author{T.~Nosek}
\affiliation{\Charles}

%For first publication
%\author{J.~Nowak}
%\affiliation{\Minnesota}

\author{Y.~Oksuzian}
\affiliation{\Virginia}

\author{A.~Olshevskiy}
\affiliation{\JINR}

%For first publication
%\author{J.~Oliver}
%\affiliation{\Harvard}

\author{T.~Olson}
\affiliation{\Tufts}

\author{J.~Paley}
\affiliation{\FNAL}

% Went legacy August 2016
%\author{P.~Pandey}
%\affiliation{\Delhi}

%For first publication
%\author{A.~Para}
%\affiliation{\FNAL}

\author{R.~B.~Patterson}
\affiliation{\Caltech}

\author{G.~Pawloski}
\affiliation{\Minnesota}

%For first publication
%\author{N.~Pearson}
%\affiliation{\Minnesota}

%For first publication
%\author{D.~Perevalov}
%\affiliation{\FNAL}

\author{D.~Pershey}
\affiliation{\Caltech}

\author{O.~Petrova}
\affiliation{\JINR}

%For first publication
%\author{E.~Peterson}
%\affiliation{\Minnesota}

\author{R.~Petti}
\affiliation{\Carolina}

\author{S.~Phan-Budd}
\affiliation{\Winona}

%For first publication
%\author{L.~Piccoli}
%\affiliation{\FNAL}

%For first publication
%\author{A.~Pla-Dalmau}
%\affiliation{\FNAL}

\author{R.~K.~Plunkett}
\affiliation{\FNAL}

% Legacy June 2017
%\author{R.~Poling}
%\affiliation{\Minnesota}

\author{B.~Potukuchi}
\affiliation{\Jammu}

\author{C.~Principato}
\affiliation{\Virginia}

\author{F.~Psihas}
\affiliation{\Indiana}


%For first publication
%\author{D.~Pushka}
%\affiliation{\FNAL}

%For first publication
%\author{X.~Qiu}
%\affiliation{\Stanford}

%Went Legacy 1 Feb 2016
%\author{N.~Raddatz}
%\affiliation{\Minnesota}

\author{A.~Radovic}
\affiliation{\WandM}

\author{R.~A.~Rameika}
\affiliation{\FNAL}


%For first publication
%\author{R.~Ray}
%\affiliation{\FNAL}

\author{B.~Rebel}
\affiliation{\FNAL}

%For first publication
%\author{R.~Rechenmacher}
%\affiliation{\FNAL}

% Legacy June 2017
%\author{B.~Reed}
%\affiliation{\SDakota}

%For first publication
%\author{R.~Reilly}
%\affiliation{\FNAL}

% Went legacy August 2016
%\author{D.~Rocco}
%\affiliation{\Minnesota}

\author{P.~Rojas}
\affiliation{\CSU}

%For first publication ?
%\author{D.~Rodkin}
%\affiliation{\INR}

%For first publication
%\author{K.~Ruddick}
%\affiliation{\Minnesota}

%For first publication
%\author{R.~Rusack}
%\affiliation{\Minnesota}

\author{V.~Ryabov}
\affiliation{\Lebedev}

\author{K.~Sachdev}
\affiliation{\FNAL}
%\affiliation{\Minnesota}

%For first publication
%\author{S.~Sahijpal}
%\affiliation{\Panjab}

%For first publication
%\author{H.~Sahoo}
%\affiliation{\ANL}

% Legacy June 2017
%\author{P.~Sail}
%\affiliation{\Texas}

\author{O.~Samoylov}
\affiliation{\JINR}

\author{M.~C.~Sanchez}
\affiliation{\Iowa}
%\affiliation{\ANL}

%For first publication
%\author{N.~Saoulidou}
%\affiliation{\FNAL}

%For first publication
%\author{Ph.~Schlabach}
%\affiliation{\FNAL}

%For first publication
%\author{J.~Schneps}
%\affiliation{\Tufts}

% Legacy June 2017
%\author{R.~Schroeter}
%\affiliation{\Harvard}

\author{J.~Sepulveda-Quiroz}
\affiliation{\Iowa}
%\affiliation{\ANL}

\author{P.~Shanahan}
\affiliation{\FNAL}

% Went legacy August 2016
%\author{I.~Shandrov}
%\affiliation{\JINR}

%For first publication
%\author{B.~Sherwood}
%\affiliation{\Minnesota}

%Early year request
\author{A.~Sheshukov}
\affiliation{\JINR}

% Legacy June 2017
%\author{J.~Singh}
%\affiliation{\Panjab}

% Legacy June 2017
%\author{J.~Singh}
%\affiliation{\Jammu}

\author{P.~Singh}
\affiliation{\Delhi}

\author{V.~Singh}
\affiliation{\BHU}

%For first publication
%\author{A.~Smith}
%\affiliation{\Minnesota}

%Went Legacy 1 Sep 2015
%\author{D.~Smith}
%\affiliation{\SDakota}

%Added June 2017
\author{E.~Smith}
\affiliation{\Indiana}

\author{J.~Smolik}
\affiliation{\CTU}

\author{P.~Snopok}
\affiliation{\IIT}

\author{N.~Solomey}
\affiliation{\WSU}

\author{E.~Song}
\affiliation{\Virginia}

%For first publication
%\author{A.~Sotnikov}
%\affiliation{\JINR}

\author{A.~Sousa}
\affiliation{\Cincinnati}

\author{K.~Soustruznik}
\affiliation{\Charles}

%For first publication
%\author{Y.~Stenkin}
%\affiliation{\INR}

%For first publication; but rejoined January 2017
\author{M.~Strait}
\affiliation{\Minnesota}

\author{L.~Suter}
%\affiliation{\ANL}
\affiliation{\FNAL}

\author{R.~L.~Talaga}
\affiliation{\ANL}

% Went legacy August 2016
%\author{M.~C.~Tamsett}
%\affiliation{\Sussex}

%For first publication
%\author{S.~Tariq}
%\affiliation{\FNAL}

\author{P.~Tas}
\affiliation{\Charles}

% Asked to be removed in December 2016
%\author{R.~J.~Tesarek}
%\affiliation{\FNAL}

\author{R.~B.~Thayyullathil}
\affiliation{\Cochin}

\author{J.~Thomas}
\affiliation{\UCL}

%For first publication
%\author{K.~Thomsen}
%\affiliation{\Duluth}

%Went Legacy 1 Aug 2016
%\author{X.~Tian}
%\affiliation{\Carolina}

\author{E.~Tiras}
\affiliation{\Iowa}

\author{S.~C.~Tognini}
\affiliation{\UFG}

%Went Legacy 1 Feb 2016
%\author{R.~Toner}
%\affiliation{\Harvard}

\author{D.~Torbunov}
\affiliation{\Minnesota}

%For first publication
%\author{J.~Trevor}
%\affiliation{\Caltech}

\author{J.~Tripathi}
\affiliation{\Panjab}

%Added March 2017
\author{A.~Tsaris}
\affiliation{\FNAL}

\author{Y.~Torun}
\affiliation{\IIT}

%For first publication
%\author{G.~Tzanakos}
%\altaffiliation{\deceased}
%\affiliation{\Athens}

\author{J.~Urheim}
\affiliation{\Indiana}

\author{P.~Vahle}
\affiliation{\WandM}

\author{J.~Vasel}
\affiliation{\Indiana}

%For first publication
%\author{L.~Valerio}
%\affiliation{\FNAL}

%Went Legacy 1 January 2018 opted in
\author{L.~Vinton}
\affiliation{\Sussex}

\author{P.~Vokac}
\affiliation{\CTU}

\author{A.~Vold}
\affiliation{\Minnesota}

\author{T.~Vrba}
\affiliation{\CTU}

%For first publication
%\author{A.~V.~Waldron}
%\affiliation{\Sussex}

%Went Legacy 1 January 2018 opted in
\author{B.~Wang}
\affiliation{\SMU}

%Went Legacy 1 Feb 2016
%\author{Z.~Wang}
%\affiliation{\Virginia}

\author{T.K.~Warburton}
\affiliation{\Iowa}

%For first publication
% Remember to remove Oxford and RAL
%\author{A.~Weber}
%\affiliation{\Oxford}
%\affiliation{\RAL}


%For first publication
%\author{A.~Wehmann}
%\affiliation{\FNAL}

\author{M.~Wetstein}
\affiliation{\Iowa}

\author{D.~Whittington}
\affiliation{\Syracuse}
\affiliation{\Indiana}

%For first publication
%\author{N.~Wilcer}
%\affiliation{\FNAL}

%For first publication
%\author{R.~Wildberger}
%\affiliation{\Minnesota}


%For first publication
%\author{A.~Wildman}
%\altaffiliation{\deceased}
%\affiliation{\FNAL}

%For first publication
%\author{K.~Williams}
%\affiliation{\FNAL}

\author{S.~G.~Wojcicki}
\affiliation{\Stanford}

\author{J.~Wolcott}
\affiliation{\Tufts}

%For first publication
%\author{K.~Wood}
%\affiliation{\ANL}

%For first publication
%\author{M.~Xiao}
%\affiliation{\FNAL}

% Went legacy August 2016
%\author{T.~Xin}
%\affiliation{\Iowa}

%Went legacy Jan 2018
%\author{N.~Yadav}
%\affiliation{\Guwahati}

\author{S.~Yang}
\affiliation{\Cincinnati}

\author{S.~Yu}
\affiliation{\ANL}
\affiliation{\IIT}

%Went Legacy 1 Feb 2016
%\author{S.~Zadorozhnyy}
%\affiliation{\INR}

\author{J.~Zalesak}
\affiliation{\IOP}

\author{B.~Zamorano}
\affiliation{\Sussex}

%For first publication
%\author{A.~Zhao}
%\affiliation{\ANL}

%Went Legacy 1 Feb 2016
%\author{J.~Zirnstein}
%\affiliation{\Minnesota}

\author{R.~Zwaska}
\affiliation{\FNAL}

\collaboration{The NOvA Collaboration}
\noaffiliation

\date{\today}

%\maketitle

%\end{document}

